Synthetic 3D Data Generation Pipeline for Geometric Deep Learning in Architecture

With the growing interest in deep learning algorithms and computational design in the architectural field, the need for large, accessible and diverse architectural datasets increases. We decided to tackle this problem by constructing a field-specific synthetic data generation pipeline that generates an arbitrary amount of 3D data along with the associated 2D and 3D annotations. The variety of annotations, the flexibility to customize the generated building and dataset parameters make this framework suitable for multiple deep learning tasks, including geometric deep learning that requires direct 3D supervision. Creating our building data generation pipeline we leveraged architectural knowledge from experts in order to construct a framework that would be modular, extendable and would provide a sufficient amount of class-balanced data samples. Moreover, we purposefully involve the researcher in the dataset customization allowing the introduction of additional building components, material textures, building classes, number and type of annotations as well as the number of views per 3D model sample. In this way, the framework would satisfy different research requirements and would be adaptable to a large variety of tasks. All code and data are made publicly available.

==> GeometricDeepLearning/DeepLearningFramework.tex <==
\section{Geometric Deep Learning Framework}
Learning-based 3D reconstruction works are based on different 3D representations as presented before. While voxel representations prove to be computationally expensive, point cloud representations are demonstrated to be rotation and translation invariant, and computationally more efficient than voxels \cite{pointvoxcnn19}, and few parametrical representations have been researched ( important approach in architecture for building envelope design) \cite{pienet20}. Moreover, mesh representations, preserve the connections between distinct parts better and result more suitable for fine-grain detailed representations. In the end, modern implicit functions proved to be not only extremely efficient with their continuous and differentiable representation of the iso-surface with binary value representation of inside and outside points, but also more accurate for such tasks as reconstruction and 3D shape completion \cite{gu2020weaklysupervised}. Therefore, Nerf \cite{mildenhall2020nerf}, Occupancy Network\cite{occupancynet18}, DeftTef \cite{DefTet20} have recently followed for this task and are supported by the open source community ( Nerf and Implicit function supported in Pytorch3d \cite{pytorch3d20}. 

 
Within the AEC, 3D shapes and objects preserve a common grammar \cite{shapegrammar20}, are composed by a fixed set of components such as windows, doors, roof, floors, walls, and others \cite{3dscenegraph19}. While the typology can change, the main elements in the building stay the same for most cases (except for some iconic buildings and pavilions). The philosophy of Hoffman and Richards influenced this research. In fact, they viewed object recognition tasks as a visual system decomposition of shapes into parts with their descriptions and spatial relations. In the same way, we propose that the best way of representing a building is to assemble each component together, orienting their quaternions to perfectly fit an initial picture. Furthermore, our work was inspired by the CompoNet work \cite{componet}. In contrast to the approach, we aim to translate the assembly algorithm, specifically for an an architectural task. They used a generative neural network for generating 3D shapes from a 2D image, based on a part-based prior, where the key idea was for the network to synthesize shapes by varying both the shape parts and their compositions. Treating a shape not as an unstructured whole, but as a composable set of deformable parts, adds a combinatorial dimension to the generative process to enrich the diversity of the output, encouraging the generator to venture more into the “unseen”. They generated a plethora of shapes compared with baseline generative models using their custom metrics. We did not explore so in depth the composition of our buildings, we limited this research on assembly specific elements, without deforming singular components. This assembly-based synthesis was inspired by 3d shape assembly research that generates new shapes from a combination of various parts \cite{huang2020generative3dpartass}, \cite{li19pargenassstruct}. In our case, we are not exploring the generation of novel and new building but a 3d reconstruction from a single image, that can benefit from these previous conversations.  


\subsection{Proposed framework}

After perusing previous related research, we propose a two-fold framework: the first step recognizes the object and the second step converts it to a 3D representation (3D Reconstruction Framework).  

We considered all possible 3D representation formats to perform a perfect training: orderless point clouds (PointNET \cite{pointnet16}, \cite{sauder19}), voxels (VoxNET, oct-trees, \cite{voxnet15} ), RGBD projected view, multi-view depth maps, surface meshes (volumetric representations (References), primitive-based CAD models ( reference) or implicit functions ( NeRF \cite{mildenhall2020nerf}), and others. This heterogeneity provided limitations to define a unified approach. Not only different representations but also different techniques have been adopted in the past for an optimal 3D reconstruction: multi-view \cite{tulsiani18multiview}, single-view approaches, or hybrid (3D-R2N2 \cite{3dr2n216}). Even though multi-view approaches related to shape retrieval tasks \cite{zou20} boast higher levels of accuracy, we focused on mostly hybrid representations starting from a single view with implicit functions and point clouds. Not only, the single image approaches can scale to a multi-view one \cite{mildenhall2020nerf} improving its performance with the addition of RNN, LSTM or Transformers and other techniques, that can translate a series of images into a sequence or a 3D representations of 3D models, but it is also more democratic and practical. Since we operated on a single image, we were able to perform instance segmentation, object detection, and shape retrieval operations easily by using current state of the art algorithms such as MaskRCNN \cite{maskrcnn20} (using the Detectron2 framework), obtaining a perfect segmentation of the building envelope. This first part of the 3D reconstruction workflow is a fundamental one for the establishment of this framework. Once we are capable to isolate the object that we want to translate in 3d, many different solutions that involved differentiable render will become more accessible and easier to use.  In fact, for our exploration we used tools such as Kaolin, PyTorch3D \cite{pytorch3d20}, PyTorch Geometric, PyT Geom Temporal and others to perform these tests.  In this second part of the framework, we identify its strict link to recognition inferences of the parts or components that constitute the building such as walls, doors, windows, balconies, roofs, chimneys. This operation can be performed with semantic, topology, synthesis, structure (StructEdit\cite{partnet20}[46]) features. Instead of encoding shapes as points in the latent space, representing shape differences (SD) as vectors, some approaches used SD as primary objects and encode them in their own latent space with a conditional variational autoencoder (CVAE) in order to generalize better also in shapes that are not on the training set, as optimal for our use case. Shapes should encode in terms of fine-grained part with a Hierarchical Semantic Segmentations (StructureNET \cite{structedit19}, GRASS\cite{structnet19}, Im2Struct \cite{im2struct18},\textcolor{red}{we need to fix here!} OccNet \cite{occupancynet18},\cite{convoccnet20},\cite{deepoctreeWang20}), in fact, encoding SD enables dealing with inhomogeneities in the shape space thanks to different combinatorial part structures of the PartNET dataset \cite{mopartnetdataset20} and other unsupervised approaches from an image \cite{rezende16} .  Other methods with Structure-aware shape synthesis \cite{li19pargenassstruct} proved their limitations with fine-grained parts for part assembly. A more robust method with a hierarchical part organization is needed (3D Part Assembly\cite{partnet20} or Scores \cite{scores18}) without the generalization provided by learning their primitive's shapes \cite{learnshapeabst17}. After reproducing these approaches, we discovered that unsupervised techniques for unseen objects and parts using a shape to program \cite{tian193dshapeprog} approach worked quite well. Moreover, learning 3D Part Assembly from a Single Image \cite{partnet20} , using a U-Net with an encoder-decoder architecture helped with an Image-guided shaped structure decoding. It was the key to solve this problem. The approach is based on Geometric Deep Learning \cite{geometricdeeplearning17} used successfully in combination with a graph embedding network, 3D CGAN, with non-Euclidean Reimann geometry (Reimann Manifold) and with Ensemble CNNs \cite{ensemblecnn20}. We identify the best approach as a compositional one, that for the lack of resources at the current moment, it was impossible to fully develop and test.  

 
We base our current framework for the 3D reconstruction as a positioning one related to how the building facades are assembled, with pose estimation in a 6D space (3D rotation, and translation vector aligning part center in the camera space). It is optimal to assemble the building components (with adjacency graph convolutions) instead of completely reconstructing them. We can take advantages from their repetitive pattern, similarities, and symmetries.  

 Finally, given a single RGBD image it translates to a 3D object and a set of different 3D part point clouds. The goal of the function was to predict a set of poses for the objects. The network architecture was categorized by different modules: one with the image segmentation mask, and one where 2D and 3D features are combined for predicting the pose of the objects using quaternions. Another step is related to the normalization of the dimensions, preserving their scales. Then identical parts can be clustered together improving its efficiency. Specific loss functions that take in consideration chamfer distance, EMD, spherical interpolation, projections, and other metrics were implemented. Moreover, for the placement and positioning of obscured parts unsupervised approaches can be further tested. Shape to program algorithms could allowed to weight different property such as symmetry (chair with 4 legs where 2 occluded the picture \cite{tian193dshapeprog}). Furthermore, Local Deep Implicit Function (LDIF) and Unsupervised 3D Learning for Shape Analysis via Multiresolution Instance Discrimination  \cite{wang2021unsupervised} allowed to generalize better and is capable to recognize more granular and detailed shapes and is not constrained by the training set. In this way it would be possible to associate a latent vector to its regions specific for each sub part.  

 


